Model-Agnostic Meta Learning for Differentiable MPC

Applying policy optimization to Model Predictive Control (MPC) yields high-performance and reliable controllers. However, the resulting controllers often overfit their training conditions and suffer significant performance degradation in unseen tasks. We propose a novel framework combining policy optimization with meta-learning to train highly adaptable MPC controllers. Our approach enables rapid adaptation to unseen tasks, maintaining high performance at a fraction of the computational cost required for full retraining. Furthermore, we integrate system identification into the pipeline to continuously refine both the MPC hyperparameters and the underlying predictive models. We validate our proposed methodology on a Ball-on-Plate system, demonstrating superior adaptability across various parameterized trajectory-tracking tasks.

==> Figures/controller_comparison/circle.tex <==
\def\datafile{CCcircle.dat}

\begin{tikzpicture}
\begin{axis}[
  width=\linewidth,
  axis equal image,
  xlabel={Position $x$ (m)},
  ylabel={Position $y$ (m)},
  grid=both,
  legend pos=north east,
  % Discards coordinates that fail the filter instead of plotting lines to the origin
  unbounded coords=discard 
]

\addplot[
    blue4, 
    line width=1.2pt,
    restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}
]
table[col sep=space, x=x, y=y]{\datafile};
\addlegendentry{Nominal MPC (SysID)}

\addplot[
    orange1, 
    dash dot, 
    line width=1.0pt,
    restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==1}{1:1}
]
table[col sep=space, x=x, y=y]{\datafile};
\addlegendentry{LQR (SysID)}

\addplot[
    yellow1, 
    dotted, 
    line width=1.0pt,
    restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==2}{1:1}
]
table[col sep=space, x=x, y=y]{\datafile};
\addlegendentry{PID}

\addplot[
    green1, 
    dashed, 
    line width=1.1pt,
    restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==3}{1:1}
]
table[col sep=space, x=x, y=y]{\datafile};
\addlegendentry{Reference}

\end{axis}
\end{tikzpicture}

==> Figures/controller_comparison/square.tex <==
\def\datafile{CCsquare.dat}

\begin{tikzpicture}
\begin{axis}[
  width=\linewidth,
  axis equal image,
  xlabel={Position $x$ (m)},
  % ylabel={Position $y$ (m)},
  grid=both,
  % legend pos=north east,
  % Discards coordinates that fail the filter instead of plotting lines to the origin
  unbounded coords=discard 
]

\addplot[
    blue4, 
    line width=1.2pt,
    restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}
]
table[col sep=space, x=x, y=y]{\datafile};
% \addlegendentry{Nominal MPC (SysID)}

\addplot[
    orange1, 
    dash dot, 
    line width=1.0pt,
    restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==1}{1:1}
]
table[col sep=space, x=x, y=y]{\datafile};
% \addlegendentry{LQR (SysID)}

\addplot[
    yellow1, 
    dotted, 
    line width=1.0pt,
    restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==2}{1:1}
]
table[col sep=space, x=x, y=y]{\datafile};
% \addlegendentry{PID}

\addplot[
    green1, 
    dashed, 
    line width=1.1pt,
    restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==3}{1:1}
]
table[col sep=space, x=x, y=y]{\datafile};
% \addlegendentry{Reference}

\end{axis}
\end{tikzpicture}

==> Figures/metatrained/circle.tex <==
\def\datafile{METAcircle.dat}

\begin{tikzpicture}
\begin{axis}[
  width=\linewidth,
  xlabel={Iteration $k$},
  ylabel={Cost $\mathcal{C}(p)$},
  grid=both,
  legend pos=north east
]

% series 0
\addplot[blue4, mark=o, line width=1pt, 
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};
\addlegendentry{BP-MPC (nominal)}

% series 1
\addplot[green1, dashed, mark=x, line width=1pt, restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==1 }{1:1}]
table[col sep=space, x=x, y=y]{\datafile};
\addlegendentry{BP-MPC (meta-initialized)}

\end{axis}
\end{tikzpicture}

==> Figures/metatrained/figure_eight.tex <==
\def\datafile{METAfigure8.dat}

\begin{tikzpicture}
\begin{axis}[
  width=\linewidth,
  xlabel={Iteration $k$},
  % ylabel={Cost $\mathcal{C}(p)$},
  grid=both,
  % legend pos=north east
]

% series 0
\addplot[blue4, mark=o, line width=1pt, 
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};
% \addlegendentry{BP-MPC (nominal)}

% series 1
\addplot[green1, dashed, mark=x, line width=1pt, restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==1 }{1:1}]
table[col sep=space, x=x, y=y]{\datafile};
% \addlegendentry{BP-MPC (meta-initialized)}

\end{axis}
\end{tikzpicture}

==> Figures/metatrained/square.tex <==
\def\datafile{METAsquare.dat}

\begin{tikzpicture}
\begin{axis}[
  width=\linewidth,
  xlabel={Iteration $k$},
  % ylabel={Cost $\mathcal{C}(p)$},
  grid=both,
  % legend pos=north east
]

% series 0
\addplot[blue4, mark=o, line width=1pt, 
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};
% \addlegendentry{BP-MPC (nominal)}

% series 1
\addplot[green1, dashed, mark=x, line width=1pt, restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==1 }{1:1}]
table[col sep=space, x=x, y=y]{\datafile};
% \addlegendentry{BP-MPC (meta-initialized)}

\end{axis}
\end{tikzpicture}

==> Figures/sys_id_comparison/circle.tex <==
\def\datafile{SIcircle.dat}

\begin{tikzpicture}
\begin{axis}[
  width=\linewidth,
  xlabel={Iteration $k$},
  ylabel={Cost $\mathcal{C}(p)$},
  grid=both,
  legend pos=north east
]

% series 0: BP-MPC (SysID)  [base curve]
\addplot[blue4, mark=o, line width=1pt,
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};
\addlegendentry{BP-MPC (SysID)}

% series 1: BP-MPC (no SysID)
\addplot[red3, dashed, mark=triangle*, line width=1pt,
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==1}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};
\addlegendentry{BP-MPC (no SysID)}

% series 2: BP-MPC (offline ID)
\addplot[green1, dash dot, mark=x, line width=1pt,
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==2}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};
\addlegendentry{BP-MPC (offline ID)}

\end{axis}
\end{tikzpicture}

==> Figures/tracking_error/circle.tex <==
\def\datafile{TEcircle.dat}

\begin{tikzpicture}
\begin{axis}[
  width=\linewidth,
  % xlabel={Iteration $k$},
  ylabel={Tracking error $e$},
  grid=both
]

% series 0: BP-MPC tracking error curve
\addplot[blue4, mark=o, line width=1pt,
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};

% series 1: boxplot data around p0 iteration
\addplot[gray, mark=none, line width=0.9pt,
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==1}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};

% series 2: boxplot data around pbest iteration
\addplot[black, dashed, mark=none, line width=0.9pt,
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==2}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};

\end{axis}
\end{tikzpicture}

==> Figures/tracking_error/square.tex <==
\def\datafile{TEsquare.dat}

\begin{tikzpicture}
\begin{axis}[
  width=\linewidth,
  xlabel={Iteration $k$},
  ylabel={Tracking error $e$},
  grid=both
]

% series 0: BP-MPC tracking error curve
\addplot[blue4, mark=o, line width=1pt,
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};

% series 1: boxplot data around p0 iteration
\addplot[gray, mark=none, line width=0.9pt,
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==1}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};

% series 2: boxplot data around pbest iteration
\addplot[black, dashed, mark=none, line width=0.9pt,
restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==2}{1:1}]
table[col sep=space, x=x, y=y]{\datafile};

\end{axis}
\end{tikzpicture}

==> Figures/trajectory_plots/trajectory_plots.tex <==
\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group size=3 by 1,
        horizontal sep=1.5cm,
    },
    width=7cm,%\linewidth,
    axis equal image,
    grid=both,
    xlabel={\small Position $x$ (m)},
    ylabel={\small Position $y$ (m)},
    unbounded coords=discard,
    legend cell align={center},
    legend columns=-1,
    legend style={at={(1.75,1.05)}, anchor=south, draw=none, /tikz/every even column/.append style={column sep=10pt}}
]

% Left Plot (Circle Trajectories)
\nextgroupplot

% Initial BP-MPC: Dash-Dot
\addplot[red3, dashdot, line width=2.0pt, restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}] 
table[col sep=space, x=x, y=y]{xycircle.dat};
\addlegendentry{Untrained MPC}

% SysID MPC: Solid
\addplot[blue4, line width=2.0pt, restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}] 
table[col sep=space, x=x, y=y]{CCcircle.dat};
\addlegendentry{SysID MPC}

% Converged BP-MPC: Dotted
\addplot[green1, dotted, line width=2.5pt, restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==1}{1:1}] 
table[col sep=space, x=x, y=y]{xycircle.dat};
\addlegendentry{BP-MPC}

% Reference: Dashed
\addplot[black, dashed, line width=1.1pt, restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==2}{1:1}] 
table[col sep=space, x=x, y=y]{xycircle.dat};
\addlegendentry{Reference}

% Middle Plot (Square Trajectories)
\nextgroupplot[ylabel={}]

% Initial BP-MPC
\addplot[red3, dashdot, line width=2.0pt, restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}] 
table[col sep=space, x=x, y=y]{xysquare.dat};

% SysID MPC
\addplot[blue4, line width=2.0pt, restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==0}{1:1}] 
table[col sep=space, x=x, y=y]{CCsquare.dat};

% Converged BP-MPC
\addplot[green1, dotted, line width=2.5pt, restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==1}{1:1}] 
table[col sep=space, x=x, y=y]{xysquare.dat};

% Reference
\addplot[black, dashed, line width=1.1pt, restrict expr to domain={\thisrow{axis_id}==0 && \thisrow{series_id}==2}{1:1}] 
table[col sep=space, x=x, y=y]{xysquare.dat};

% Right Plot (The Image) - Limits set to fill the plot area
\nextgroupplot[hide axis, xmin=0, xmax=1, ymin=0, ymax=1]
\addplot graphics [xmin=0, xmax=1, ymin=0, ymax=1] {joint.png};

\end{groupplot}
\end{tikzpicture}
